VM14K: First Vietnamese Medical Benchmark

Medical benchmarks are indispensable for evaluating the capabilities of language models in healthcare for non-English-speaking communities,therefore help ensuring the quality of real-life applications. However, not every community has sufficient resources and standardized methods to effectively build and design such benchmark, and available non-English medical data is normally fragmented and difficult to verify. We developed an approach to tackle this problem and applied it to create the first Vietnamese medical question benchmark, featuring 14,000 multiple-choice questions across 34 medical specialties. Our benchmark was constructed using various verifiable sources, including carefully curated medical exams and clinical records, and eventually annotated by medical experts. The benchmark includes four difficulty levels, ranging from foundational biological knowledge commonly found in textbooks to typical clinical case studies that require advanced reasoning. This design enables assessment of both the breadth and depth of language models' medical understanding in the target language thanks to its extensive coverage and in-depth subject-specific expertise. We release the benchmark in three parts: a sample public set (4k questions), a full public set (10k questions), and a private set (2k questions) used for leaderboard evaluation. Each set contains all medical subfields and difficulty levels. Our approach is scalable to other languages, and we open-source our data construction pipeline to support the development of future multilingual benchmarks in the medical domain.

==> figures/diagram_pipeline.tex <==

%----start diagram data pipeline----
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300
%Shape: Rectangle [id:dp06394154647275174] 
\draw   (3,159) -- (156.8,159) -- (156.8,199) -- (3,199) -- cycle ;
%Rounded Rect [id:dp6425461090400781] 
\draw   (174,17) .. controls (174,12.58) and (177.58,9) .. (182,9) -- (236,9) .. controls (240.42,9) and (244,12.58) .. (244,17) -- (244,41) .. controls (244,45.42) and (240.42,49) .. (236,49) -- (182,49) .. controls (177.58,49) and (174,45.42) .. (174,41) -- cycle ;
%Shape: Rectangle [id:dp3089237819512689] 
\draw   (330.8,8.6) -- (490.8,8.6) -- (490.8,64.6) -- (330.8,64.6) -- cycle ;
%Shape: Rectangle [id:dp0072620438286810085] 
\draw   (181.8,160) -- (283.8,160) -- (283.8,200) -- (181.8,200) -- cycle ;
%Shape: Rectangle [id:dp5392433653488999] 
\draw   (300,160) -- (385.8,160) -- (385.8,200) -- (300,200) -- cycle ;
%Straight Lines [id:da9835936647257364] 
\draw    (155.8,99.6) -- (82.37,157.36) ;
\draw [shift={(80.8,158.6)}, rotate = 321.81] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5410278130628179] 
\draw    (206.8,57.6) -- (212.8,79.6) ;
%Straight Lines [id:da9699512497336178] 
\draw    (217.8,101.6) -- (232.31,158.66) ;
\draw [shift={(232.8,160.6)}, rotate = 255.74] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da08002909329566887] 
\draw    (206.8,57.6) -- (235.8,80.6) ;
%Straight Lines [id:da1562861058385716] 
\draw    (259.8,100.6) -- (334.23,159.36) ;
\draw [shift={(335.8,160.6)}, rotate = 218.29] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9498491255242769] 
\draw    (206.8,57.6) -- (179.8,80.6) ;
%Straight Lines [id:da33884347425225236] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (416.8,65.6) -- (158.68,158.32) ;
\draw [shift={(156.8,159)}, rotate = 340.24] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8982873717828399] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (416.8,65.6) -- (285.43,158.84) ;
\draw [shift={(283.8,160)}, rotate = 324.63] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6483375535991462] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (416.8,65.6) -- (386.42,158.1) ;
\draw [shift={(385.8,160)}, rotate = 288.18] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da22119708353543777] 
\draw    (206.8,57.6) -- (328.83,36.93) ;
\draw [shift={(330.8,36.6)}, rotate = 170.39] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Snip Single Corner Rect [id:dp9092119583845446] 
\draw   (76,244) -- (109.67,244) -- (127.8,262.13) -- (127.8,297.03) -- (76,297.03) -- cycle ;
%Snip Single Corner Rect [id:dp4396951850260502] 
\draw   (413.8,255) -- (502.8,255) -- (516.8,269) -- (516.8,295) -- (413.8,295) -- cycle ;
%Snip Single Corner Rect [id:dp448135562010205] 
\draw   (248.06,245) -- (291.24,245) -- (309.8,263.56) -- (309.8,298.03) -- (248.06,298.03) -- cycle ;
%Straight Lines [id:da47363513833182624] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (127.8,262.13) -- (156.8,262.6) ;
%Straight Lines [id:da11013196609003462] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (215.8,261.6) -- (242.8,262.53) ;
\draw [shift={(244.8,262.6)}, rotate = 181.97] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da49659985292138] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (309.8,263.56) -- (323.8,263.6) ;
%Straight Lines [id:da569559361446146] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (387.8,264.6) -- (411.8,264.6) ;
\draw [shift={(413.8,264.6)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da3650278919722525] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (45.8,264.6) -- (72.8,264.6) ;
\draw [shift={(74.8,264.6)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da1378837919814233] 
\draw    (59.8,200.6) -- (30.88,245.91) ;
\draw [shift={(29.8,247.6)}, rotate = 302.55] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9136029769001781] 
\draw    (219.8,200.6) -- (210.22,245.64) ;
\draw [shift={(209.8,247.6)}, rotate = 282.01] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5890741988629624] 
\draw    (343.8,200.6) -- (358.17,243.7) ;
\draw [shift={(358.8,245.6)}, rotate = 251.57] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% Text Node
\draw (188,22) node [anchor=north west][inner sep=0.75pt]   [align=left] {admin};
% Text Node
\draw (307,172) node [anchor=north west][inner sep=0.75pt]   [align=left] {EL service};
% Text Node
\draw (4,83) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{225.54pt}\setlength\topsep{0pt}
\begin{center}
The administrator create and manage all via APIs
\end{center}
\end{minipage}};
% Text Node
\draw (191.08,172) node [anchor=north west][inner sep=0.75pt]   [align=left] {spark cluster};
% Text Node
\draw (16,171) node [anchor=north west][inner sep=0.75pt]   [align=left] {extract data service};
% Text Node
\draw (160,256) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{45.8pt}\setlength\topsep{0pt}
\begin{center}
transform
\end{center}
\end{minipage}};
% Text Node
\draw (330,257) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{37.31pt}\setlength\topsep{0pt}
\begin{center}
transfer
\end{center}
\end{minipage}};
% Text Node
\draw (4,258) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{26.53pt}\setlength\topsep{0pt}
\begin{center}
crawl
\end{center}
\end{minipage}};
% Text Node
\draw (335,17.84) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{101.95pt}\setlength\topsep{0pt}
\begin{center}
airflow orchestral\\(schedule and trigger)
\end{center}
\end{minipage}};
% Text Node
\draw (415.8,267.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {Hugging Face};
% Text Node
\draw (82.82,252) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{25.95pt}\setlength\topsep{0pt}
\begin{center}
S3\\(raw)
\end{center}
\end{minipage}};
% Text Node
\draw (250.13,253) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{40.71pt}\setlength\topsep{0pt}
\begin{center}
S3\\(bronze)
\end{center}
\end{minipage}};
\end{tikzpicture}
%----end diagram data pipeline----

==> tables/accuracy_by_difficulties.tex <==


\begin{table}[]
\centering
\begin{tabular}{lcccc}
                  & \textbf{Easy}   & \textbf{Medium} & \textbf{Challenging} & \textbf{All}    \\ \hline
claude-3-5-sonnet & 0.7433          & 0.7109          & 0.7178               & 0.7205          \\ \hline
deepseek-r1       & \textbf{0.8241} & \textbf{0.7895} & \textbf{0.7759}      & \textbf{0.7976} \\ \hline
gemini-2-0-flash  & 0.7966          & 0.7582          & 0.7165               & 0.7644          \\ \hline
gpt-4o            & 0.7560          & 0.7247          & 0.6903               & 0.7297          \\ \hline
llama4-maverick   & 0.7313          & 0.7192          & 0.7040               & 0.7209          \\ \hline
o3-mini           & 0.7365          & 0.7155          & 0.6833               & 0.7179          \\ \hline
qwen3             & 0.7495          & 0.7166          & 0.7042               & 0.7243          \\ \hline
\end{tabular}
\caption{Accuracy of different models with simple prompt}
\label{tab:foundation-pass-at-1}
\end{table}



\begin{table}[]
\centering
\begin{tabular}{lcccc}
                      & \textbf{Easy}   & \textbf{Medium} & \textbf{Challenging} & \textbf{All}    \\ \hline
claude-3-5-sonnet-agg & 0.7471          & 0.7196          & 0.7275               & 0.7279          \\ \hline
deepseek-r1-agg       & \textbf{0.8311} & \textbf{0.7904} & \textbf{0.7663}      & \textbf{0.7990} \\ \hline
gemini-2-0-flash-agg  & 0.8056          & 0.7592          & 0.7303               & 0.7689          \\ \hline
gpt-4o-agg            & 0.7713          & 0.7321          & 0.7202               & 0.7416          \\ \hline
llama4-maverick-agg   & 0.7384          & 0.7268          & 0.7220               & 0.7293          \\ \hline
o3-mini-agg           & 0.7451          & 0.7187          & 0.6801               & 0.7219          \\ \hline
qwen3-agg             & 0.7628          & 0.7258          & 0.6994               & 0.7332          \\ \hline
\end{tabular}
\caption{Accuracy of different models - ensemble 3 runs with shuffled options}
\label{tab:foundation-ensemble-with-shuffle}
\end{table}

==> tables/performance_by_topic_pass_at_3.tex <==

\begin{table}[]
\caption{Pass@3 accuracy of the foundation models. Values are accuracies in percentages.}
\label{tab:foundation-pass-at-3}
\vspace{5pt}
\centering
\begin{tabular}{lcccc}
\toprule
                         & \textbf{Easy}   & \textbf{Medium} & \textbf{Challenging} & \textbf{All}    \\
\midrule
Claude 3.5 Sonnet        & 77.50          & 74.81          & 74.43               & 75.62          \\ 
Deepseek-R1              & \textbf{84.68} & \textbf{82.32} & \textbf{82.31}      & \textbf{83.02} \\ 
Gemini Flash 2.0         & 80.16          & 77.34          & 74.77               & 77.92          \\ 
GPT-4o                   & 82.78          & 79.57          & 77.95               & 80.40          \\ 
Llama4 Maverick          & 74.68          & 72.66          & 71.17               & 73.13          \\ 
\bottomrule
\end{tabular}
\end{table}

==> tables/performance_overall.tex <==

\begin{table}[]
\centering
\caption{Overall accuracy of different foundation models: Pass@1 vs. Ensemble. Values are accuracies in percentages.}
\vspace{5pt}
\begin{tabular}{lccc}
\toprule
                  & \textbf{Pass@1} & \textbf{Ensemble} & \textbf{Improvement} \\ 
\midrule
Claude 3.5 Sonnet & 71.46      & 72.31    & 0.85    \\ 
Deepseek-R1       & \textbf{78.17}          & \textbf{78.42}             & 0.25    \\ 
Gemini-2-0-Flash  & 75.67      & 76.30    & 0.63    \\ 
GPT-4o            & 72.74      & 73.80    & \textbf{1.07}        \\ 
Llama4 Maverick   & 71.76      & 72.46    & 0.70    \\ 
o3-mini           & 71.42      & 72.02    & 0.60    \\ 
Qwen3-32B         & 72.47      & 73.40    & 0.93    \\ 
\bottomrule
\end{tabular}
\label{tab:foundation-accuracy}
\end{table}


